Potenziali di Evans su variet\`a paraboliche

This is my master thesis. Unfortunately it is written in Italian, but maybe somebody will find it helpful when it comes to Evans Potentials

==> char_roy.tex <==
\subsection{Esempi non banali di caratteri}\label{sec_charroy}
Come preannunciato nel capitolo \ref{chap_filtri}, utilizziamo gli ultrafiltri e in particolare i risultati ottenuti nella sezione \ref{sec_charsucc} per descrivere alcuni caratteri non banali sull'algebra di Royden (quindi punti di $R^*$).\\
Dalla definizione di carattere, ci si aspetta che sull'algebra di Royden esistano dei caratteri che in qualche senso rappresentino il limite della funzione in una certa direzione. Ad esempio se consideriamo una successione $x_n\in R$, l'operazione di limite lungo questa successione è un'operazione lineare e moltiplicativa su $\Ro$ quando definita, nel senso che date due funzioni $f$ e $g$ tali che esista il limite $\lim_n f(x_n)$ e $\lim_n g(x_n)$, allora vale che:
\begin{gather*}
 \lim_n (f\cdot g)(x_n)=\lim_n f(x_n) \cdot \lim_n g(x_n)
\end{gather*}
data una funzione in $\Ro$, non sempre è garantito che su ogni successione che tende a infinito esista il limite di $f(x_n)$. Per aggirare questo problema, utilizziamo i limiti lungo ultrafiltri.
\begin{oss}
 Con la tecnica mostrata nella sezione \ref{sec_charsucc} è possibile definire caratteri anche sulle algebre di Royden. Basta considerare una qualsiasi successione $\{x_n\}$ in $R$ e un qualsiasi ultrafiltro $\M$ su $\N$ e definire
\begin{gather*}
 \phi(f)=\lim_{\M} f(x_n)
\end{gather*}
Se l'ultrafiltro è non costante, allora $\phi$ è un'operazione di limite, quindi:
\begin{gather*}
 \liminf_n f(x_n)\leq \phi(f)\leq \limsup_n f(x_n)
\end{gather*}
Questo garantisce che l'operazione descritta sia un'estensione dell'operazione di limite standard, nel senso che se esiste $\lim_n f(x_n)$, allora $\phi(f)=\lim_n f(x_n)$, e anche che questo carattere non sia un carattere banale, non sia cioè un carattere immagine attraverso $\tau$ di un punto di $R$. Infatti è sempre possibile creare una funzione in $\Ro$ che valga $1$ su un qualsiasi punto fissato $\bar x$ e che valga $O$ definitivamente su una successione $x_n$ che tende a infinito \footnote{quindi $\phi(f)=0$, mentre $\bar x(f)\equiv f(\bar x) =1$}.\\
La compattificazione di Royden quindi contiene tutti i caratteri che rendono conto del comportamento di una funzione al ``limite'' lungo una successione.
\end{oss}
In realtà non è necessario passare attraverso le successioni, con un ragionamento molto simile a quello sviluppato nella sezione precendente, si osserva che
\begin{prop}
 Ogni ultrafiltro $\M$ su $R$ definisce un carattere sull'algebra di Royden, quindi un elemento di $R^*$
\begin{proof}
 La dimostrazione è la generalizzazione della dimostrazione di \ref{prop_car_N}.
Consideriamo una funzione continua limitata $f:R\to \R$. La collezione $f(\M)$ è un ultrafiltro in $\R$, anzi un ultrafiltro in $[\inf_{R}(f),\sup_R(f)]$, insieme compatto. Quindi per ogni funzione possiamo definire
\begin{gather*}
 \phi_{\M}(f)=\lim f(\M)
\end{gather*}
e con argomenti del tutto analoghi alla dimostrazione \ref{prop_car_N} ottenere che $\phi$ è un carattere su $M(R)$.
\end{proof}
\end{prop}
Quello che manca in questo caso rispetto a sopra è la proprietà che vale per gli ultrafiltri non costanti
\begin{gather*}
 \liminf_n x(n) \leq \phi(x) \leq \limsup_n x(n)
\end{gather*}
quindi una specie di controllo del carattere con il comportamento di $f$ all'infinito. Ovviamente non ha senso la definizione standard di $\liminf$ e $\limsup$ per una funzione che come dominio ha un'insieme con la potenza del continuo, ma comunque anche in questo caso esiste una proprietà simile, che verrà esplorata nella sezione successiva.

==> dirichlet.old.tex <==
\section{Problema di Dirichlet}
In questa sezione tratteremo la risolubilità del problema di Dirichlet su particolari domini su varietà Riemanniane. Lo scopo della sezione è ottenere risultati tecnici che saranno utilizzati in futuro per la tesi, citando i risultati noti e cercando di dimostrare risultati particolari con tecniche il più elementari possibili.\\
Introdurremo come prima cosa il problema di Dirichlet, citando alcuni casi in cui è risolubile con facilità (ad esempio il caso in cui il dominio abbia bordo liscio). Con la caratterizzazione dei punti regolari del bordo data dal metodo delle barriere cercheremo di estendere questi risultati a casi più generali e grazie all'equivalenza tra la risolubilità del problema di Dirichlet con particolari operatori ellittici e il laplaciano standard su domini in $\R^n$ dimostreremo con una tecnica relativamente elementare che il problema di Dirichlet si può risolvere anche su domini solitamente non considerati nella letteratura standard.\\
In tutta la sezione $\Omega$ indicherà un dominio in $R$ o in $\R^n$, cioè un insieme aperto connesso relativamente compatto, e $L$ indicherà un operatore strettamente ellittico del secondo ordine con $c=0$ (il laplaciano su varietà differenziali soddisfa queste ipotesi).
\subsection{Domini con bordo liscio}
\begin{deph}
 Dato un dominio $\Omega\subset R$, un operatore ellittico del secondo ordine $L:C^2(R)\to C(R)$ e una funzione continua $\phi:\partial \Omega \to \R$, diciamo che $\Phi$ è soluzione del problema di Dirichlet
\begin{gather*}
 L(\Phi)=0 \ \ su \ \ \Omega\\
\Phi|_{\partial \Omega}=\phi
\end{gather*}
se $\Phi\in C^2(\Omega)\cap C(\overline \Omega)$ e soddisfa le condizioni appena enunciate.
\end{deph}
La solubilità del problema di Dirichlet è fortemente legata alla regolarità del dominio $\Omega$. Ad esempio, se $\Omega=B(0,1)\setminus \{0\}\subset \R^n$ \footnote{$B(0,1)$ indica la bolla di raggio $1$ in $\R^n$}, non esistono soluzioni del problema di Dirichlet uguali a $0$ sul bordo di $B(0,1)$ e diverse da $0$ ma limitate nell'origine (vedi esercizi 15 e 16 cap 3 pag 57 di \cite{24}, e per un altro esempio vedi es 25 cap 2 pag 54 dello stesso libro).\\
Per illustrare i primi casi in cui il problema di Dirichlet ammette un'unica soluzione, introduciamo alcune definizioni.
\begin{deph}
 Un dominio $\Omega\subset R$ ha bordo $C^k$ con $0\leq k\leq \infty$ se e solo se per ogni punto $p\in \partial \Omega$, esiste un intorno $V(p)$ e una funzione $f\in C^k(V,\R)$ tale che:
\begin{gather*}
 \Omega \cap V = f^{-1}(\infty,0) \ \ \ \partial \Omega \cap V =f^{-1}(0)
\end{gather*}
\end{deph}
Osserviamo che non è sufficiente per un dominio in $R$ avere il bordo costutuito da sottovarietà regolari per essere considerato di bordo liscio. Ad esempio se $\Omega$ è una bolla in $R$ a cui togliamo una sottovarietà regolare con bordo $S$ contenuta nella bolla, non è un dominio regolare. Infatti per ogni punto $p\in S^{\circ}$ esiste un intorno $V(p)$ e una funzione liscia tale che $S\cap V=f^{-1}(0)$, ma non è vero che $\Omega\cap V =f^{-1}(-\infty,0)$, infatti $\Omega\cap V=f^{-1}(\{0\}^C)$.\\
Per domini con bordo sufficientemente liscio.

==> titlepage.tex <==
\begin{titlepage}

\begin{center}
UNIVERSIT\`A DEGLI STUDI DELL'INSUBRIA
\end{center}

\begin{center}
 

\ 
Dipartimento di scienze MM. FF. NN. Como \\
Anno accademico 2008 - 2009\\
Sessione di laurea del 30 Settembre 2009\\

\ \newline
{\Huge 

Tesi di Matematica: \\
}
\ \\

\Huge{\textbf{Potenziali di Evans\\ su varietà paraboliche}}

\ \newline
\newline
\includegraphics[width=.5\textwidth]{logo}
\end{center}

\begin{flushright}
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
\newline
Autore:\\

Daniele Valtorta, matricola 617528\\
e-mail: \href{mailto:danielevaltorta@gmail.com}{danielevaltorta@gmail.com}
\\

Relatore:\\

Alberto Giulio Setti\\

Corelatore:\\

Stefano Pigola\\

\end{flushright}
\end{titlepage}
